Probing the Robustness of Vision-Language Pretrained Models: A Multimodal Adversarial Attack Approach

Vision-language pretraining (VLP) with transformers has demonstrated exceptional performance across numerous multimodal tasks. However, the adversarial robustness of these models has not been thoroughly investigated. Existing multimodal attack methods have largely overlooked cross-modal interactions between visual and textual modalities, particularly in the context of cross-attention mechanisms. In this paper, we study the adversarial vulnerability of recent VLP transformers and design a novel Joint Multimodal Transformer Feature Attack (JMTFA) that concurrently introduces adversarial perturbations in both visual and textual modalities under white-box settings. JMTFA strategically targets attention relevance scores to disrupt important features within each modality, generating adversarial samples by fusing perturbations and leading to erroneous model predictions. Experimental results indicate that the proposed approach achieves high attack success rates on vision-language understanding and reasoning downstream tasks compared to existing baselines. Notably, our findings reveal that the textual modality significantly influences the complex fusion processes within VLP transformers. Moreover, we observe no apparent relationship between model size and adversarial robustness under our proposed attacks. These insights emphasize a new dimension of adversarial robustness and underscore potential risks in the reliable deployment of multimodal AI systems.

==> biography.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio/guan.jpeg}}]{Jiwei Guan} received the Master Research degree from Macquarie University, Sydney, NSW, Australia. In 2019, he was a research engineer in the Cyber-Physical Systems Group from CSIRO data61, Brisbane, QLD, Australia. He is currently pursuing a Ph.D.~degree with Macquarie University and CSIRO Data61 Software \& Computational Systems Group, Sydney, NSW, Australia. His research interests focus on trustworthy machine learning, interpretable AI, multimodal fusion, multimodal robustness, and natural language processing. He specializes in dialogue systems and harvesting robotics.
\end{IEEEbiography}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio/pan.jpg}}]{Lei Pan} 
received the Ph.D.~degree in computer forensics from Deakin University, Australia, in 2008. He is currently a Senior Lecturer with the Centre for Cyber Resilience and Trust (CREST), School of Information Technology, Deakin University. He leads the research theme `Securing Data and Infrastructure' at CREST. His research interests cover broad topics in cybersecurity and privacy. He has authored 100 research papers in refereed international journals and conferences, such as IEEE Transactions on Information Forensics and Security, IEEE Transactions on Dependable and Security Computing, IEEE Transactions on Industrial Informatics, and many more.
\end{IEEEbiography}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio/wang.jpg}}]{Chen Wang} received his Ph.D.~in Computer Science from Nanjing University. He is currently a principal research scientist at CSIRO Data61, Australia. His current research interests are on the interpretability, robustness and scalability of data-driven systems. He leads and develops machine learning and data analytics systems for various domains, including radio astronomy, health, and agriculture as well as smart grids. He is a member of the ACM.
\end{IEEEbiography}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio/yu.png}}]{Shui Yu} (IEEE F'23) obtained his PhD from Deakin University, Australia, in 2004. He is a Professor of School of Computer Science, University of Technology Sydney, Australia. His research interest includes Cybersecurity, Network Science, Big Data, and Mathematical Modelling. He has published five monographs and edited two books, more than 500 technical papers at different venues, such as IEEE TDSC, TPDS, TC, TIFS, TMC, TKDE, TETC, ToN, and INFOCOM. His current h-index is 66. Professor Yu promoted the research field of networking for big data since 2013, and his research outputs have been widely adopted by industrial systems, such as Amazon cloud security. He is currently serving the editorial boards of IEEE Communications Surveys and Tutorials (Area Editor) and IEEE Internet of Things Journal (Editor). He served as a Distinguished Lecturer of IEEE Communications Society (2018--2021). He is a Distinguished Visitor of IEEE Computer Society, and an elected member of Board of Governors of IEEE VTS and ComSoc, respectively. He is a member of ACM and AAAS, and a Fellow of IEEE.
\end{IEEEbiography}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio/gao.jpg}}]
\end{IEEEbiography}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio/zheng.jpg}}]{Xi Zheng} received the Ph.D. in Software Engineering from the University of Texas at Austin in 2015. From 2005 to 2012, he was the Chief Solution Architect for Menulog Australia. He is currently the Director of Intelligent Systems Research Group (ITSEG.ORG), Director of International engagement in the School of Computing, Senior Lecturer (equivalent to Associate Professor US) and Deputy Program Leader in Software Engineering, Macquarie University, Australia. His research interests include Cyber-Physical Systems Testing and Verification, Safety Analysis, Distributed Learning, Internet of Things, and Software Engineering in general. He has secured more than \$1.2 million competitive funding in Australian Research Council (Linkage and Discovery) and Data61 (CRP) projects on safety analysis, model testing and verification, and trustworthy AI on autonomous vehicles. He also won a few awards including Deakin Industry Researcher (2016) and MQ Earlier Career Researcher (Runner-up 2020). He has a number of highly cited papers and best conference papers. He served as PC members for Software and System flagship conferences including FSE (2022) and PerCom (2017--2023). He also served as the PC chairs of IEEE CPSCom-2021, IEEE Broadnets-2022 and associate editor for ACM Distributed Ledger Technologies.
\end{IEEEbiography}

